Interacting Hopf Algebras: the theory of linear systems

As first main contribution, this thesis characterises the PROP SVk of linear subspaces over a field k - an important domain of interpretation for circuit diagrams appearing in diverse research areas. We present by generators and equations the PROP IH of string diagrams whose free model is SVk. IH stands for interacting Hopf algebras: its equations arise by distributive laws between Hopf algebras, which we obtain using Lack's technique for composing PROPs. The significance of the result is two-fold. First, it offers a canonical diagrammatic syntax for linear algebra: linear maps, kernels, subspaces, etc... are all faithfully represented in the graphical language. Second, the equations of IH describe familiar algebraic structures - Hopf algebras and Frobenius algebras - which are at the heart of graphical formalisms as seemingly diverse as quantum circuits, signal flow graphs, simple electrical circuits and Petri nets. Our characterisation enlightens the provenance of these axioms and reveals their linear algebraic nature. Our second main contribution is an application of IH to the semantics of signal processing circuits. We develop a formal theory of signal flow graphs, featuring a diagrammatic circuit syntax, a structural operational semantics and a denotational semantics. We prove completeness of the equations of IH for denotational equivalence. Also, we study full abstraction: it turns out that the purely operational picture is too concrete - two denotationally equal graphs may exhibit different operational behaviour. We classify the ways in which this can occur and show that any graph can be realised - rewritten, using the equations of IH, into an executable form where the operational behaviour and the denotation coincide. This realisability theorem suggests a reflection about the role of causality in the semantics of signal flow graphs and, more generally, of computing devices.

==> source/background/propoperations.tex <==
We present three different ways of combining PROPs: sum (coproduct), sequential composition and fibered sum (pushout). We shall use these operations to understand PROPs \emph{modularly}, as the result of the interaction of simpler components.

%These techniques are particularly useful to canonically obtain presentations by generators and equations: the idea is to split up a given PROP $\T$ as the result of operations on simpler PROPs for which an equational presentation is known, and then use this information to construct the SMT for $\T$. 

==> source/chapterHOPF/BackgroundHOPF.tex <==
\paragraph{Notation} Composition of arrows $f \: a \to b$, $g\: b \to c$ is denoted by $f\poi g \: a \to c$. $\catC[a,b]$ indicates the set of arrows from $a$ to $b$ in a small category $\catC$. For $\catC$ symmetric monoidal, we use notation $\tns$ for the monoidal product and $\sigma_{X,Y} \: X \tns Y \to Y \tns X$ for the symmetry associated with $X,Y \in \catC$. Given $\funF \: \catC_1 \to \catC_2$, we denote with $\funF^{\op} \: \catC_1^{\op}\to \catC_2^{\op}$ the induced functor on the opposite categories of $\catC_1, \catC_2$. Given $\catC$ with pullbacks, its span bicategory has the objects of $\catC$ as $0$-cells, spans of arrows of $\catC$ as $1$-cells and span morphisms as $2$-cells. We denote with $\Span{\catC}$ the category obtained by identifying the isomorphic $1$-cells and forgetting the $2$-cells. Dually, if $\catC$ has pushouts we can form its bicategory of cospans and denote with $\Cospan{\catC}$ the category obtained by identifying the isomorphic $1$-cells and forgetting the $2$-cells.


\subsection{PROPs}\label{ssec:propsbackground}

A one-sorted \emph{symmetric monoidal theory} (SMT) is determined by a pair $(\Sigma, E)$ where $\Sigma$ is the \emph{signature}: a set of \emph{generators} $o \: n\to m$ with \emph{arity} $n$ and \emph{coarity} $m$. The set of $\Sigma$-terms is obtained by composing generators in $\Sigma$, the unit $\id \: 1\to 1$ and the symmetry $\sigma_{1,1} \: 2\to 2$ with $;$ and $\tns$. This is a purely formal process: given $\Sigma$-terms $t \: k\to l$, $u \: l\to m$, $v \: m\to n$, we construct new $\Sigma$-terms $t \mathrel{;} u \: k\to m$ and $t \tns v \: k+n \to l+n$.  The set $E$ of \emph{equations} contains pairs of $\Sigma$-terms of the form $(t,t':k\to l)$; here the only requirement is that $t$ and $t'$ have the same arity and coarity as $\Sigma$-terms.

SMTs are presentations of PROPs~\cite{MacLane1965,Lack2004a} (product and permutation categories). A PROP is a strict symmetric monoidal category with objects natural numbers, where $\tns$ on objects is addition. Morphisms between PROPs are strict symmetric monoidal functors that are identity on objects: PROPs and their morphisms form the category $\PROP$.
Now, given an SMT $(\Sigma,E)$, one (freely) obtains a PROP by letting the arrows $k\to l$ be the set of $\Sigma$-terms $k\to l$ taken modulo the laws of symmetric monoidal categories and the (smallest congruence containing the) equations $t=t'$ for any $(t,t')\in E$. There is a natural graphical representation of these terms as arrows of monoidal categories (see~\cite{Selinger2009}): we will commonly refer to these diagrams, which can be considered as $\Sigma$-terms modulo the laws of (strict) monoidal categories, as \emph{circuits}.

For example, let $(\Sigma_M,E_M)$ be the SMT of commutative monoids. The signature $\Sigma_M$ contains two generators:  multiplication --- which we depict as a circuit $\Wmult \: 2 \to 1$ --- and unit, represented as $\Wunit \: 0 \to 1$.
 Graphically, the generation of $\Sigma_M$-terms amounts to ``tiling'' $\Wmult$ and $\Wunit$ together with the circuit $\symNet$ (representing $\sigma_{1,1}\: 2 \to 2$) and $\Idnet$ (representing $\id_1 \: 1 \to 1$). Equations $E_M$ assert associativity \eqref{eq:wmonassoc}, commutativity \eqref{eq:wmoncomm} and identity \eqref{eq:wmonunitlaw}.
 \begin{multicols}{3}\noindent
\begin{equation}
\label{eq:wmonunitlaw}
\tag{A1}
\lower11pt\hbox{$\includegraphics[height=1cm]{graffles/Wunitlaw.pdf}$}
\!\!\!
=\!
\lower5pt\hbox{$\includegraphics[height=.6cm]{graffles/idcircuit.pdf}$}
\end{equation}
\begin{equation}
\label{eq:wmoncomm}
\tag{A2}
\lower5pt\hbox{$\includegraphics[height=.6cm]{graffles/Wmult.pdf}$}
\!
=
\!\!\!\!
\lower11pt\hbox{$\includegraphics[height=1cm]{graffles/Wcomm.pdf}$}
\end{equation}
\begin{equation}
\label{eq:wmonassoc}
\tag{A3}
\lower12pt\hbox{$\includegraphics[height=1cm]{graffles/Wassocl.pdf}$}
\!\!\!
=
\!\!\!
\lower12pt\hbox{$\includegraphics[height=1cm]{graffles/Wassocr.pdf}$}
\end{equation}
\end{multicols}
We call $\wmon$ the PROP freely generated by the SMT $(\Sigma_M,E_M)$.\footnote{The notation $w$ emphasizes the white colouring of circuits in $\Sigma_M$ --- later on, we will use the black colouring for another copy of the same PROP.}

For later reference, we also introduce the PROP $\bcom$ of (black) cocommutative comonoids, generated by the signature consisting of circuits $\Bcomult$, $\Bcounit$ and the following equations.
\begin{multicols}{3}\noindent
\begin{equation}
\label{eq:bcomonunitlaw}
\tag{A4}
\lower11pt\hbox{$\includegraphics[height=1cm]{graffles/Bcounitlaw.pdf}$}
\!\!\!
=
\!
\lower7pt\hbox{$\includegraphics[height=.7cm]{graffles/idcircuit.pdf}$}
\end{equation}
\begin{equation}
\label{eq:bcomoncomm}
\tag{A5}
\lower5pt\hbox{$\includegraphics[height=.6cm]{graffles/Bcomult.pdf}$}
\!
=
\!\!\!
\lower11pt\hbox{$\includegraphics[height=1cm]{graffles/Bcomm.pdf}$}
\end{equation}
\begin{equation}
\label{eq:bcomonassoc}
\tag{A6}
\lower11pt\hbox{$\includegraphics[height=1cm]{graffles/Bcoassocl.pdf}$}
\!\!\!
=
\!\!\!
\lower11pt\hbox{$\includegraphics[height=1cm]{graffles/Bcoassocr.pdf}$}
\end{equation}
\end{multicols}

Modulo the white vs. black colouring, the circuits of $\bcom$ can be seen as those of $\wmon$ ``reflected about the $y$-axis''. This observation yields that $\bcom \cong (\wmon {})^{op}$. More generally, for $\T$ a PROP freely generated from an SMT, $\T^{op}$ can be presented by generators and equations which are those of $\T$ reflected about the $y$-axis.

We will sometimes refer to the free PROPs which arise from SMTs --- e.g.\ to the examples above --- as \emph{syntactic} PROPs in order to distinguish them from \emph{semantic} PROPs that are defined ``directly'': an example of a semantic PROP is the PROP $\F$ where arrows $k\to l$ are simply functions $\{0,\dots, k-1\}\to \{0, \dots, l-1\}$. Note that this is purely an issue of presentation: indeed,
%A useful observation is that $\F$ provides a ``concrete'' representation of the SMT of commutative monoids:
 there is an isomorphism $\wmon \cong \F$ which amounts to considering a circuit $c \in \wmon[n,m]$ as the graph of a function of type $\{0,\dots, n-1\}\to \{0, \dots, m-1\}$. For instance, $\Wmult \tns \Wunit \: 2 \to 2$ describes the function $f \: \{0,1\} \to \{0,1\}$ mapping both elements to $0$.

As observed by Lack~\cite{Lack2004a}, PROPs can also be seen as objects of a certain coslice category. To illustrate this, we need the concept of PRO, generalising the one of PROP: it is a strict monoidal (i.e.\ not necessarily symmetric) category with objects the natural numbers and tensor product on objects being addition. The morphisms of PROs are strict monoidal functors that are identity on objects. There is a PRO of particular interest: the PRO of permutations $\Perm$, where the homset $\Perm[k,l]$ is empty if $k\neq l$ and otherwise contains all the permutations on the set with $k$ elements. PROPs can now be understood as objects of the slice category $\mathbb{P}/\PRO$, where $\PRO$ is the category of PROs and their morphisms. Morphisms of PROPs are thus simply morphisms of PROs that preserve the permutation structure. Working in the slice is also intuitive: e.g. $\mathbb{P}$ is the initial PROP and in order to compute the coproduct $\mathbb{T}_1+\mathbb{T}_2$ in $\PROP$ one must identify the permutation structures in $\mathbb{T}_1$ and $\mathbb{T}_2$. A useful observation is that, if $\mb{T}_1$ is presented by the SMT $(\Sigma_1,E_1)$ and $\mb{T}_2$ by $(\Sigma_2,E_2)$, then $\mb{T}_1 + \mb{T}_2$ is presented by the disjoint union of theories $(\Sigma_1 \uplus \Sigma_2, E_1\uplus E_2)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Composing PROPs}\label{ssec:composingPROP}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The sum $\mb{T}_1 + \mb{T}_2$ is not the only way in which theories can be combined together. Instead, one usually is interested to study the quotient of $\mb{T}_1 + \mb{T}_2$ by some equations, expressing a compatibility condition between $\mb{T}_1$ and $\mb{T}_2$. This situation describes a typical pattern in algebra: for instance, a ring is given by a monoid and an abelian group, subject to equations telling how the former structure distributes over the latter. Similarly, the laws of bialgebras can be seen as arising by the interaction of a monoid and a comonoid. In~\cite{Lack2004a} Lack shows how this phenomenon can be understood as the operation of composing together two PROPs to form a more complex theory.

We now detail how PROP composition is formally expressed in terms of distributive laws between monads. As shown in the classical work \cite{Street_MonadsI} of Street, the theory of monads can be developed in an arbitrary bicategory. In this perspective, small categories are just monads in $\Span{\Set}$. Similarly, PROPs can be described as monads on $\mathbb{P}$ in the bicategory $\mathsf{Prof}(\mathbf{Mon})$ of strict monoidal categories and profunctors~\cite{Lack2004a}.

Now, any two PROPs $\T_1$ and $\T_2$ can be composed via a distributive law $\lambda \colon \T_2 \poi \T_1 \to \T_1  \poi \T_2$ between the associated monads. $\lambda$ makes $\T_1 \poi  \T_2$ into a monad, yielding a PROP whose arrows can be seen as \emph{pairs} $(f,g) \: n \to m$, where $f \: n \to z$ is an arrow of $\T_1$ and $g \: z \to m$ one of $\T_2$.
%
A key observation for our purposes is that the graph of $\lambda$ can be also seen as a set of (directed) equations of the form $(g,f) = (f',g')$. In fact, if $\T_1$ and $\T_2$ are syntactic PROPs then $\T_1 \poi  \T_2$ also has a presentation by generators and equations: this is the same as the coproduct $\T_1 +  \T_2$, plus the equations encoded by $\lambda$. This fits the intuition given above: $\T_1 \poi  \T_2$ is the sum of theories $\T_1$ and $\T_2$ subject to the compatibility conditions expressed by the distributive law.


As an example, we show how composing the PROPs $\bcom$ and $\wmon$ of commutative comonoids and monoids yields the PROP of co/commutative bialgebras. First observe that circuits of $\bcom$ correspond to arrows of $\Fop$, because $\bcom \cong (\wmon {})^{\op} \cong \F^{\op}$. We can then express a distributive law $\lambda \: \wmon \poi \bcom \To \bcom \poi \wmon$ as having the type $\F \poi \Fop \To \Fop \poi \F$, that is, it maps a pair $p \in \F[n,z]$, $q \in \Fop[z,m]$ to a pair $f \in \Fop[n,z]$, $g \in \F[z,m]$. This amounts to saying that $\lambda$ maps \emph{cospans} $n \tr{p} z \tl{q} m$ into \emph{spans} $n \tl{f} r \tr{g} m$ in $\F$. Defining $n \tl{f} r \tr{g} m$ as the pullback of $n \tr{p} z \tl{q} m$ makes indeed $\lambda$ satisfy the equations of distributive laws~\cite{Lack2004a}. The resulting PROP $\bcom \poi \wmon$ can be presented by generators --- the ones of $\bcom + \wmon$ --- and equations --- the ones of $\bcom + \wmon$ together with those given by the graph of $\lambda$. By definition of $\lambda$, one can read them (in $\bcom + \wmon$) out of the pullback squares in $\F$. For instance:
\noindent \begin{minipage}{8cm}
\begin{eqnarray*}
\xymatrix@R=12pt@C=15pt{
& 1 & && & & 1 \ar[dr]^{\sem{\bcom}^{-1}(\initVect_1)} &\\
\ar[ur]^{\finVect} 2 & & 0 \ar[ul]_{\initVect_1} & \ar@{|=>}[r] & & \ar[ur]^{\sem{\wmon}^{-1}(\finVect)} 2 \ar[dr]_{\sem{\bcom}^{-1}(\initVect_2)} & & 0 \\
& \ar[ul]^{\initVect_2} 0 \pullbackcorner \ar[ur]_{\id_0} & & && & 0 \ar[ur]_{\sem{\wmon}^{-1}(\id_0)} & }
\end{eqnarray*}
\end{minipage}
\begin{minipage}{7cm}
yields $\Wmult ; \Bcounit = \twoBcounit \poi \id_0$
\end{minipage}
\smallskip

\noindent
where $\finVect\: 2 \to 1$ and $\initVect_n \: 0 \to n$ are given, respectively, by finality of $1$ and initiality of $0$ in $\F$, and $\sem{\wmon} \: \wmon \xrightarrow{\cong}\F$, $\sem{\bcom} \: \bcom \xrightarrow{\cong}\Fop$ are the isomorphisms. In fact, all the equations presenting $\bcom \poi \wmon$ can be derived from (those of $\bcom + \wmon$ and) just four pullback squares  (\emph{cf.} \cite[\S 5.3]{Lack2004a}) that yield:
\begin{multicols}{2}
\noindent
\begin{equation}
\label{eq:unitsl}
\lower2pt\hbox{$
\tag{A7}
\lower5pt\hbox{$\includegraphics[height=.6cm]{graffles/lunitsl.pdf}$}
=
\lower5pt\hbox{$\includegraphics[height=.6cm]{graffles/lunitsr.pdf}$}
$}
\end{equation}
\begin{equation}
\label{eq:unitsr}
\tag{A9}
\lower5pt\hbox{$\includegraphics[height=.6cm]{graffles/runitsl.pdf}$}
=
\lower5pt\hbox{$\includegraphics[height=.6cm]{graffles/runitsr.pdf}$}
\end{equation}
\begin{equation}
\label{eq:bialg}
\tag{A8}
\lower6pt\hbox{$\includegraphics[height=.6cm]{graffles/bialgl.pdf}$}
=
\lower11pt\hbox{$\includegraphics[height=.9cm]{graffles/bialgr.pdf}$}
\end{equation}
\begin{equation}
\label{eq:bwbone}
\tag{A10}
\lower4pt\hbox{$\includegraphics[height=.5cm]{graffles/unitsl.pdf}$}
=
\ \ \id_0\phantom{\quad}
\end{equation}
\end{multicols}
 Therefore $\bcom \poi \wmon$ is the free PROP of (black-white) co/commutative bialgebras, obtained as the quotient of $\bcom + \wmon$ by \eqref{eq:unitsl}-\eqref{eq:bwbone}. As another perspective on the same result, one can say that the PROP of co/commutative bialgebras is the theory of $\Span{\F} \cong \Fop \poi \F$ and each circuit $c \: n \to m$ of this PROP can be factorised as $c = c_1\poi c_2$, where $c_1 \in \bcom[n,z]$ and $c_2 \in \wmon[z,m]$ for some $z$.

There is a dual characterisation for $\Cospan{\F}$. The distributive law, of type $\bcom \poi \wmon\To \wmon\poi \bcom$, is defined by pushout in $\F$. Its equations are presented by the PROP of \emph{separable Frobenius algebras}~\cite{Carboni1987}. We refer to~\cite{Lack2004a} for the details. Interestingly, the Frobenius equations will also appear in our development (Section~\ref{sec:ibrw}), though for different reasons.


\begin{comment}
\subsection{Computing the Kernel of Matrices over a PID}\label{sec:HNF}

\input{./source/3_Hermite}

\subsection{Categories of Matrices over a PID}\label{sec:catmatrices}

In this section we set up a categorical environment for $\PID$-matrices. First, we fix notation for the following categories:
\begin{itemize}
  \item the abelian category $\RMod{\PID}$ of $\PID$-modules and linear maps;
  \item its full subcategory $\FRMod{\PID}$ consisting of the finitely-generated free $\PID$-modules and linear maps between them;
  \item the PROP $\VectR$ with arrows $n\to m$ being $m\times n$ $\PID$-matrices, where $;$ is matrix multiplication and $\tns$ is direct sum. The permutations are the rearrangements of the rows of the identity matrix.
\end{itemize}

There is an equivalence of categories between $\FRMod{\PID}$ and $\VectR$: a finitely-generated free $\PID$-module in $\FRMod{\PID}$, say of dimension $n$, is isomorphic to $\PID^n$ and thus we can associate it with the object $n$ in $\VectR$. A linear map $f \: V \to W$ in $\FRMod{\PID}$ is represented by a matrix $M \: n \to m$, where $V \cong \PID^n$ and $W \cong \PID^m$.

As $\FRMod{\PID}$ has biproducts given by direct sum, in $\VectR$ the object $n + m$ is the biproduct of $n$ and $m$. Given two matrices $A \: n \to z$ and $B \: m \to z$ in $\VectR$, we denote with $(A|B) \: n + m \to z$ the matrix given by the universal property of $n + m$ as coproduct. Dually, given matrices $C \: z \to n$ and $D \: z \to m$, $(\frac{C}{D}) \: z \to n + m$ is the matrix given by the universal property of $n + m$ as product. The graphical notation reflects the way in which these matrices are constructed, by putting $A$ and $B$ side-by-side and $C$ above $D$.

For our purposes, it is of importance to discuss the existence of pullbacks and pushouts in $\VectR$. Two matrices $A \: n \to z$ and $B \: m \to z$ in $\VectR$ can be represented in $\RMod{\PID}$ as arrows of type $\PID^n \to \PID^z$ and $\PID^m \to \PID^z$. Since $\RMod{\PID}$ is an abelian category, their pullback may be formed by calculating the kernel $\Ker{A|-B} \: V \to \PID^n \tns \PID^m$. %(see e.g. \cite[Tag 00ZU]{stacks-project}).
Now, it is a well-known fact that (assuming the axiom of choice) $\PID$ is a PID iff every submodule of a free $\PID$-module is itself free. The kernel object $V$ is a submodule of $\PID^n \tns \PID^m$ and therefore $V \cong \PID^r$ for some natural number $r \leq n+m$. We can then express the pullback of $A$ and $B$ in $\RMod{\PID}$ as follows:
\[\xymatrix@C=40pt@R=35pt{
&\ar[dl]_{C} \PID^r \ar[d]|{\Ker{A|-B}} \ar[dr]^{D} & \\
\PID^n \ar[dr]_{A}  & \PID^n \tns \PID^m \ar[d]|{(A|-B)} & \PID^m \ar[dl]^{B} \\
& \PID^z  & }\]
Since $\Ker{A|-B}$ ranges over $\PID^n \tns \PID^m$, it is of shape $(\frac{C}{D}) \: \PID^r \to \PID^n \tns \PID^m$ and postcomposition with the product projections $\pi_1 \: n \tns m \to n$ and $\pi_2 \: n \tns m \to m$ yields matrices $C$ and $D$ as in the diagram. It follows that we also have a pullback square in $\VectR$:
\[\xymatrix@=10pt{
&\ar[dl]_{C} r \ar[dr]^{D} & \\
n \ar[dr]_{A}  & & m \ar[dl]^{B} \\
& z  & }\]
Unfortunately, the same reasoning does not apply for pushouts. Given matrices $C \: \PID^z \to \PID^n$ and $D \: \PID^z \to \PID^m$, their pushout in $\RMod{\PID}$ is formed by taking the cokernel $\Coker{C|-D} \: \PID^n \tns \PID^m \to Q$. The object $Q$ is not necessarily a free module, meaning that we cannot see that as a pushout diagram in $\VectR$. Nonetheless, $\VectR$ \emph{does} have pushouts, because it is a self-dual category, with isomorphism $\VectR \cong \VectRop$ given by taking the transpose of a matrix. Therefore for purely formal reasons the pushout of matrices $C \: z \to n$ and $D \: z \to m$ in $\VectR$ exists as the transpose of the pullback of transposed matrices $C^T \: n \to z$ and $D^T \: m \to z$ (note that this does not, in general, coincide with the pushout in $\RMod{\PID}$).

% (i) The fact that $\PID$ is PID means that we can calculate pullbacks in the category of $\PID$-modules, because of the well-known fact that (assuming the axiom of choice) $\PID$ is a PID iff every submodule of a free module is itself free (*). Thus the forgetful functor from the category of (all) $\PID$-modules to $\Set$ creates pullbacks and since $\FRMod\PID$ embeds fully into the category of all $\PID$-modules these pullbacks, by (*), reflect to $\FRMod\PID$. Note that $\Mat{\PID}$ is self dual via the transpose operation on arrows and thus for purely formal reasons pushouts also exist in $\Mat{\PID}$ (note that pushouts in $\Mat{\PID}$, and so in $\FRMod{\PID}$, do not, in general, coincide with pushouts in the category of all $\PID$-modules!).


\subsection{From Matrices over a PID to Matrices over its Field of Fractions}\label{sec:backfieldfractions}

Given the PID $\PID$, we fix notation $\frPID$ for its field of fractions. This is canonically constructed by letting elements of $\frPID$ be fractions $\frac{k_1}{k_2}$, where $k_1 , k_2 \in \PID$, $k_2 \neq 0$ and $\frac{k_1}{k_2}$ represents an equivalence class of the relation $(k_1,k_2) \sim (k_3,k_4)$ on pairs of elements of $\PID$ defined by
\[(k_1,k_2) \sim (k_3,k_4) \text{ if } k_1\cdot k_4 = k_3 \cdot k_2 \text{.}\]

As seen in Section~\ref{sec:catmatrices}, we can construct categories $\RMod{\frPID}$, $\FRMod{\frPID}$ and $\Mat{\frPID}$. Since $\frPID$ is a field, $\FRMod{\frPID}$ is just the category of finite dimensional vector spaces over $\frPID$ and $\RMod{\frPID} \cong \FRMod{\frPID}$ because any $\frPID$-module is free. There is an obvious PROP morphism $I \: \VectR \to \Mat{\frPID}$ interpreting a matrix with entries in $\PID$ as a matrix with entries in $\frPID$. Similarly, we have an inclusion $J \: \FRMod{\PID} \to \FRMod{\frPID}$. This yields the following commutative diagram, where $\simeq$ denotes equivalence of categories.
\[
\xymatrix{
{\Mat{\PID}} \ar[d]_I \ar[r]^-{\simeq} & {\FRMod{\PID}} \ar[d]^J \\
{\Mat{\frPID}} \ar[r]_-{\simeq} & {\FRMod{\frPID}}
}
\]

In the remaining of this section we record some facts that will be used in the developments of Section~\ref{sec:cubebottom}.

\begin{lemma} \label{lem:pullbacksinmat} $I: \Mat{\PID}\to \Mat{\frPID}$ preserves pullbacks and pushouts.
\end{lemma}
\begin{proof} Because the transpose operation induces a duality in both $\Mat{\PID}$ and $\Mat{\frPID}$ (\emph{cf.} Section \ref{sec:catmatrices}), the morphism $\Mat{\PID}\to\Mat{\frPID}$ preserves pullbacks iff it preserves pushouts. It is thus enough to show that it preserves pullbacks. This can be easily be proved directly as follows. Suppose that the diagram
\begin{equation}
\label{eq:pbinmatr}
\tag{$\star$}
\vcenter{
\xymatrix@=10pt{
& {r} \ar[dl]_A \ar[dr]^B \\
{n} \ar[dr]_C & & {m} \ar[dl]^D \\
& {z}
}
}
\end{equation}
is a pullback in $\Mat{\PID}$. We need to show that it is also a pullback in $\Mat{\frPID}$.
Suppose that, for some $P \: q\to n$, $Q \: q\to m$ in $\Mat{\frPID}$ we have that
$CP = DQ$ in $\Mat{\frPID}$. Since $\PID$ is a PID we can find least common multiples:
thus let $d$ be a common multiple of all the denominators that appear in $P$ and $Q$.
Then $dP \: q \to n$, $dQ \: q\to m$ are in $\Mat{\PID}$ and we have
$C(dP)=d(CP)=d(DQ)=D(dQ)$. Since \eqref{eq:pbinmatr} is a pullback in $\Mat{\PID}$, there exists a unique $H \: q\to r$ with $AH=dP$ and $BH=dQ$. This means that we have found a mediating arrow, $H/d \: q \to r$, in $\Mat{\frPID}$ since $A(H/d)=AH/d=dP/d=P$ and similarly $B(H/d)=Q$. Uniqueness in $\Mat{\frPID}$ can also be translated in a straightforward way to uniqueness in $\Mat{\PID}$. Basically if $H'$ is another mediating morphism and $d'$ is the least common multiple of denominators in $H'$ then we must have $d'(H/d)=d'H'$ because of the universal property in $\Mat{\PID}$. Dividing both sides by $d'$ yields the required equality.
\qed\end{proof}

\begin{lemma}\label{lemma:pushoutinvect}
Let the following be a pushout diagram in $\FRMod{\frPID}$.
\[
\xymatrix@=10pt{
& {U} \ar[dl]_f \ar[dr]^g  \\
{V}\ar[dr]_p & & {W} \ar[dl]^q \\
& {T}
}
\]	
Suppose that there exist $v\in V$, $w\in W$ such that $pv=qw$.
Then there exists $u\in U$ with $fu=v$ and $gu=w$.
\end{lemma}
\begin{proof}
Pushouts in $\FRMod{\frPID} \cong \RMod{\frPID}$ can be constructed by quotienting the vector space $V+W$ by the subspace generated by $\{\,(fu,gu)\,|\,u\in U\,\}$. Thus,
if $p(v) = q(w)$ then there exists a chain $u_1,u_2,\dots,u_k$
with $f(u_1)=v$, $g(u_1)=g(u_2)$, $f(u_2)=f(u_3)$, \dots, $f(u_{k-1})=f(u_{k-1})$ and $g(u_k)=w$.
If $k=1$ then we are finished. Otherwise, to construct an inductive argument we need to consider a chain $u_1, u_2, u_3$ with $f(u_1)=v$,
$g(u_1)=g(u_2)$, $f(u_2)=f(u_3)$ and $g(u_3)=w$.
Now $f(u_1-u_2+u_3)=f(u_1)-f(u_2)+f(u_3)=v$ and
$g(u_1-u_2+u_3)=g(u_1)-g(u_2)+g(u_3)=w$, so we have reduced the size of the chain to one.
\qed\end{proof}

The proof of Lemma~\ref{lemma:pushoutinvect} relies on the fact that $\RMod{\frPID}$ reflects pushouts to $\FRMod{\frPID}$, for $\frPID$ a field. Observe that the same reasoning would not work for an arbitrary PID: as we saw in Section~\ref{sec:catmatrices}, pushouts in the category $\RMod{\PID}$ are generally different from pushouts calculated in its subcategory $\FRMod{\PID}$. %This observation actually motivates the introduction of the field of fractions of $\PID$ and the fact that the category of $\frPID$-subspaces provides the pushout object of the span $\Span{\VectR} \tl{} \VectR + \VectRop \tr{} \Cospan{\VectR}$ --- see Section \ref{sec:cubebottom}.
\end{comment} 

==> source/chapterSFG/ABR2.tex <==

In this section we commence our investigation of the denotational semantics of $\CD$. We restrict to $\FC$, to which we give a semantics in terms of matrices over $\poly$, the ring of polynomials with unknown $x$ and values over $\field$. Later, in \S\ref{sec:stream}, we will show that this is consistent with the intuitions given in Remark~\ref{remark:intuition}.

The semantic domain for $\FC$ is the PROP $\Matpoly$ where arrows $n\to m$ are $m\times n$ $\poly$-matrices. The map $\dsemHAO \: \FC \to \Matpoly$ is inductively defined as follows. For \eqref{eq:SFcalculusSyntax1}:
\begin{eqnarray}\label{eq:defsemFCpart1}
    \begin{array}{rcl}
\Bcomult &\longmapsto& \tiny{\left(%
                \begin{array}{c}
                 \!\! 1 \!\!\\
                 \!\! 1\!\!
                \end{array}\right)} \\
\Bcounit &\longmapsto&  \initVect  \\
\end{array}
&
    \begin{array}{rcl}
\Wmult  &\longmapsto&   {\scriptsize\left(%
                \begin{array}{cc}
                \!\!\!  1 \! &\!\! 1 \!\!\!
                \end{array}\right)} \\
\Wunit &\longmapsto& \finVect \\
\end{array}
&
    \begin{array}{rcl}
\scalarT &\longmapsto& {\scriptsize\left(\begin{array}{c}
                 \!\!\! k\!\!\!
                \end{array}\right)} \\
\circuitXT &\longmapsto& {\scriptsize\left( \begin{array}{c}
                 \!\!\! x\!\!\!
                \end{array}\right)}%
\end{array}
\end{eqnarray}
\noindent where $\initVect \: 0 \to 1$ and $\finVect \: 1 \to 0$ are given by initiality and finality of $0$ in $\Matpoly$. For \eqref{eq:SFcalculusSyntax3}:
\begin{eqnarray}\label{eq:defsemFCpart2}
\begin{aligned}
\ZeronetT \longmapsto id_0  \qquad
\IdnetT\! \longmapsto id_1  \qquad
\symNetT \longmapsto {\scriptsize \left(%
		\begin{array}{c c}
		  \!\! 0 & 1 \!\!\\
		  \!\! 1 & 0 \!\!	
                 \end{array}\right)}
\\
c_1\tns c_2\ \longmapsto\dsemHA{c_1} \tns \dsemHA{c_2} \qquad
c_1\poi c_2\ \longmapsto\dsemHA{c_1} \poi \dsemHA{c_2}
\end{aligned}
\end{eqnarray}
From \eqref{eq:defsemFCpart2}, it is immediate that $\dsemHAO \: \FC \to \Matpoly$ is a morphism of PROPs. Indeed $\dsemHAO$ could also have been defined as the unique PROP morphism mapping the basic components as in \eqref{eq:defsemFCpart1}. During the paper, we will introduce several semantics maps and, to be concise, we will usually adopt this second formulation.

By definition, the semantics of any 1-to-1 circuit is a polynomial in $\poly$. Conversely, for any polynomial $p = k_0 + k_1 x + k_2 x^2 + \dots + k_n x^n$, the following circuit, which hereafter we denote by $\scalarp$, has semantics $\left( p \right)$.
$$\includegraphics[width=120pt]{graffles/polyexpansion.pdf}$$

\begin{corollary}\label{prop:ab=vect}
For all circuits $c,d$ in $\FC$, $\dsemHA{c}=\dsemHA{d}$ iff $c \eqHA d$.
\end{corollary}

The previous result can be conveniently exploited also for circuits in $\FCop$. Indeed,  $\dsemHAO \: \FC \to \Matpoly$ induces the PROP morphism $\dsemHAO^{\m{op}}$ on the opposite categories, that we hereafter denote by  $\dsemHAOop\: \FCop \to \Matpoly^{\m{op}}$. The PROP $\ABpolyop$, which is presented by the operations and equations of $\ABpoly$ reflected about the $y$-axis, provides a sound and complete axiomatisation for $\dsemHAOop$.
%By taking the opposite of $\ABpoly$, $\ABpolyop$, which is presented by the same operations and equations of $\ABpoly$ but reflected about the $y$-axis, we obtain a sound and complete axiomatization for $\FCop$.

\begin{corollary}\label{prop:ab=vect}
For all circuits $c,d$ in $\FCop$, $\dsemHAop{c}=\dsemHAop{d}$ iff $c \eqHAop d$.
\end{corollary}


==> source/chapterSFG/IBR.tex <==
%Let $\frpoly$ denote the field of fractions of $\poly$.
%In this section we introduce the PROP $\IBpoly$, whose axioms describe the interaction of two $\poly$-Hopf algebras, and we show that it is isomorphic to the PROP of $\frpoly$-vector subspaces.

We now consider the task of giving a semantics to $\CD$. Recall that the semantics of a circuit in $\FC$ is a matrix, or in other words, a linear transformation. As explained in Remark~\ref{remark:intuition}, the intuition for circuits in $\FC$ is that the signal flows from left to right: left ports are inputs and right ports are outputs.

These traditional mores fail in $\CD$---indeed, only some circuits have a functional interpretation. Consider $\lccB \: 2 \to 0$: the component $\Bcounit$ accepts an arbitrary signal while $\Bmult$ ensures that the signal is equal on the two ports.
In other words, the circuit is a ``bent wire'' whose behaviour is relational: its ports are neither inputs nor outputs in any traditional sense. Indeed, the semantic domain for $\CD$ is \emph{linear relations} over $\frpoly$, the field of fractions of $\poly$.

\begin{definition}\label{DEF_SV} Let $\SVpoly$ be the following PROP:
 \begin{itemize}
   \item arrows $n\to m$ are linear relations between $\frpoly^n$ and $\frpoly^m$, that is, subspaces of $\frpoly^x \times \frpoly^m$.
   %subspaces of $\frpoly^n \times \frpoly^m$ (as a $\frpoly$-vector space).
   \item composition is relational: for subspaces
   $G=\{(u,v)\,|\,u\in\frpoly^n,v\in\frpoly^z\}$ and $H=\{(v,w)\,|\,v\in\frpoly^z,w\in\frpoly^m\}$, their composition is the subspace $\{(u,w)\,|\,\exists v. (u,v)\in G \wedge (v,w)\in H\}$.
   \item The tensor product $\tns$ on arrows is given by direct sum of spaces.
   \item The symmetries $n\to n$ are induced by bijections
    of finite sets, $\rho\, :\, n\to n$ is associated with the subspace generated by
    $\{(1_i,1_{\rho i})\}_{i \ls n}$ where $1_k$ is the binary $n$-vector
    with $1$ at the $k+1$th coordinate and $0$s elsewhere.
    For instance $\sigma_{1,1}\colon 2\to 2$ is the subspace generated by
    $\{(\matrixOneZero, \matrixZeroOne) \,,\, (\matrixZeroOne, \matrixOneZero)\}$.
 \end{itemize}
 \end{definition}

 %\begin{definition}\label{def:SemIB}\vspace{-.2cm}
    Let $[\vv_1, \dots, \vv_n]$ denote the space generated by the vectors $\vv_1 \dots \vv_n$ and $\matrixNull$ the only element of the space with dimension $0$.
    The semantic map $\dsemO \: \CD \to \SVpoly$ is the only PROP morphism mapping the components in \eqref{eq:SFcalculusSyntax1} as
\begin{eqnarray*}
 \begin{array}{rcl}
\Bcomult & \!\!\longmapsto\!\! & [(%
                \matrixOnebis,\matrixOneOne)] \\
  \Bcounit & \!\!\longmapsto\!\! & [(\matrixOnebis,\matrixNull)]
 \end{array}
&
 \begin{array}{rcl}
\Wmult & \!\!\longmapsto\!\! & [(\matrixZeroOne,\matrixOnebis),(\matrixOneZero,\matrixOnebis)]\\
\Wunit & \!\!\longmapsto\!\! & [(\matrixNull,\matrixZerobis)]
 \end{array}
&
 \begin{array}{rcl}
\scalarT & \!\!\longmapsto\!\! & [(\matrixOnebis,k)] \\
\circuitXT & \!\!\longmapsto\!\! & [(\matrixOnebis,x)] \\
 \end{array}
\end{eqnarray*}
    and for the components in \eqref{eq:SFcalculusSyntax2} is symmetric, e.g. $\Bunit$ is mapped to $[(\matrixNull,\matrixOnebis)]$.
%\end{definition}

This semantics of $\CD$ in term of subspaces is ``consistent'' with those of $\FC$ and $\FCop$ in terms of (reversed) matrices. Formally, this means the commutation of following diagram, where the horizontal arrows are the obvious embeddings.
$$\xymatrix{ \FC \ar@{^{(}->}[r] \ar[d]_{\dsemHAO} & \CD \ar[d]^{\dsemO} & \FCop \ar@{_{(}->}[l] \ar[d]^{\dsemHAOop}\\
\Matpoly \ar@{^{(}->}[r] & \SVpoly & \Matpoly^{\m{op}} \ar@{_{(}->}[l] }$$
Since $\CD$ is just $\FC+\FCop$, in order to obtain a sound and complete axiomatization for $\dsemO$, we can consider the quotient of $\ABpoly + \ABpolyop$ by laws expressing the interactions between the two Hopf algebra structures. We call the resulting PROP of \emph{interacting Hopf algebras} $\IBpoly$.


\begin{definition}\label{def:IBpoly} The PROP $\IBpoly$ is the quotient of $\CD$ by the equations of $\ABpoly$, $\ABpolyop$ and the following, where $p$ ranges over $\poly \setminus \{0\}$.%\fabio{Fix alignment of S4,S7}
 \begin{multicols}{2}\noindent
\begin{equation}
\label{eq:WFrob}
\tag{S1}
\lower15pt\hbox{$\includegraphics[height=1.1cm]{graffles/WFrobS.pdf}$}
\!\!
=
\!\!
\lower11pt\hbox{$\includegraphics[height=.8cm]{graffles/WFrobX.pdf}$}
\!\!
=
\!\!
\lower15pt\hbox{$\includegraphics[height=1.1cm]{graffles/WFrobZ.pdf}$}
\end{equation}
\begin{equation}
\label{eq:BFrob}
\tag{S2}
\lower15pt\hbox{$\includegraphics[height=1.1cm]{graffles/BFrobS.pdf}$}
\!\!
=
\!\!
\lower11pt\hbox{$\includegraphics[height=.9cm]{graffles/BFrobX.pdf}$}
\!\!
=
\!\!
\lower15pt\hbox{$\includegraphics[height=1.1cm]{graffles/BFrobZ.pdf}$}
\end{equation}
\end{multicols}
 \begin{multicols}{3}\noindent
\begin{equation}
\label{eq:lcc}
\tag{S3}
\lower8pt\hbox{$\includegraphics[height=.8cm]{graffles/lccr.pdf}$}
\!\!
=\!
\lower6pt\hbox{$\includegraphics[height=.6cm]{graffles/BccSquarer.pdf}$}
\end{equation}
\begin{equation}\label{eq:wbone}
\tag{S4}
\lower6pt\hbox{$\includegraphics[height=.6cm]{graffles/Wbonemini.pdf}$} =
\lower5pt\hbox{$\includegraphics[width=16pt]{graffles/idzerocircuit.pdf}$}
\end{equation}
 \begin{equation}\label{eq:lcm}
\tag{S5}
\hspace{-.1cm}\lower7pt\hbox{$\includegraphics[height=.7cm]{graffles/polycopolyp.pdf}$}
\!
=\!
\lower6pt\hbox{$\includegraphics[height=.6cm]{graffles/idcircuit.pdf}$}
\end{equation}
\end{multicols}
\begin{multicols}{3}\noindent
\begin{equation}
\label{eq:rcc}
\hspace{-.2cm}\tag{S6}
\lower9pt\hbox{$\includegraphics[height=.8cm]{graffles/rccl.pdf}$}
\!\!
=\!
\lower7pt\hbox{$\includegraphics[height=.6cm]{graffles/BccSquarel.pdf}$}
\end{equation}
\begin{equation}\label{eq:bbone}
\hspace{-.2cm}\tag{S7}
\lower6pt\hbox{$\includegraphics[height=.6cm]{graffles/Bbonemini.pdf}$}=
\lower5pt\hbox{$\includegraphics[width=16pt]{graffles/idzerocircuit.pdf}$}
\end{equation}
\begin{equation}\label{eq:lcmop}
\tag{S8}
\hspace{-.1cm}\lower7pt\hbox{$\includegraphics[height=.7cm]{graffles/copolypolyp.pdf}$}
\!
=\!
\lower6pt\hbox{$\includegraphics[height=.6cm]{graffles/idcircuit.pdf}$}
\end{equation}
\end{multicols}
Equations~\eqref{eq:WFrob} and \eqref{eq:BFrob} are known in the literature as \emph{Frobenius laws}~\cite{Carboni1987}. Interestingly, equations \eqref{eq:lcm} and \eqref{eq:lcmop} reflect the fact that the domain $\frpoly$ of interpretation is a field: for any non-zero polynomial $p$, the circuit $\scalarp$ has inverse $\scalarpop$ (see also the derived law~\eqref{eq:flipscalar}).
%
The notation $\antipodesquare$ replaces the antipodes $\antipode$ and $\antipodeop$: they are equal as arrows in $\IBpoly$ by virtue of \eqref{eq:lcm}. We shall write $c \eqIH d$ when $c$ and $d$ in $\CD$ are equal as arrows in $\IBpoly$.
\end{definition}
The following result states that the axioms of $\IBpoly$ characterise $\SVpoly$.
\begin{theorem}\label{thm:semanticsIBpolyIso} There is an isomorphisms of PROPs between $\IBpoly$ and $\SVpoly$.
\end{theorem}
 The proof, sketched in \S\ref{sec:cube},
 %As explained there, $\IBpoly$ can be obtained by applying composing PROP techniques.
 %This
 yields the following factorisation properties.

\begin{proposition}[Factorisation of $\CD$] \label{prop:factorisationIH} For all circuits $c$ of $\CD$, there exist circuits $c'$
in span form and $c''$ in cospan form such that $c \eqIH c' \eqIH c''$.
\end{proposition}

Since all the axioms of $\IBpoly$ are sound with respect to the denotational semantics, from the above theorem immediately follows also their completeness.
\begin{corollary}\label{prop:isoIHsoundcomplete}
For all circuits $c,d$ in $\CD$, $\dsem{c}=\dsem{d}$ iff $c \eqIH d$.
\end{corollary}

\subsection{The Structure of $\IBpoly$: Compact Closedness and Derived Laws}

For the developments of \S\ref{sec:trace} it is useful to shed light on the self-dual compact closed structure of $\IBpoly$. First, we define a sequence $\alpha_n \: 2n \to 0$ of circuits:
%The circuit $\lccB$ discussed above is mapped to $\{\big( (p,p), () \big) \mid p \in \frpoly\} \subseteq \frpoly^{2}\times\frpoly^{0}$. There are similar circuits in $\IBpoly[2n,0]$ for arbitrary $n$.
 \begin{multicols}{5}
\noindent
  \begin{eqnarray*}
       \lower18pt\hbox{$
   \alpha_0 \df \! \! \! \id_0
   $}
    \end{eqnarray*}
  \begin{eqnarray*}
       \lower18pt\hbox{$
   \alpha_1 \df \! \! \! \lower7pt\hbox{$\includegraphics[height=.7cm]{graffles/rccr.pdf}$}
   $}
    \end{eqnarray*}
  \begin{eqnarray*}
         \lower18pt\hbox{$
   \alpha_2 \df \! \! \! \lower13pt\hbox{$\includegraphics[height=1.2cm]{graffles/epsilondue.pdf}$}
      $}
   \end{eqnarray*}
     \begin{eqnarray*}
   \ \ \ \alpha_3 \df \! \! \! \lower15pt\hbox{$\includegraphics[height=1.5cm]{graffles/epsilontre.pdf}$}
   \end{eqnarray*}
     \begin{eqnarray*}
        \lower18pt\hbox{$\dots$}
   \end{eqnarray*}
    \end{multicols}
Semantically, they all behave as bent wires: for instance,  $\dsem{\alpha_1} =\{\big( (p,p), () \big) \mid p \in \frpoly\}$ and $\dsem{\alpha_2} = \{\big( (p,q,p,q), () \big) \mid p,q \in \frpoly\}$. One can define circuits from $0$ to $2n$ symmetrically, starting from $\beta_2 \df \rccB \: 0 \to 2$. Now, let $\lccn$ be notation for $\beta_n$, $\rccn$ for $\alpha_n$ and $\!\!\idncircuit\!$ for $\id_n$. As shown in \cite[\S4]{interactinghopf}, the $\beta$s and the $\alpha$s form a self-dual compact closed structure on the category $\IBpoly$, i.e.\
   \begin{equation}
  \label{eq:gensnake}
  \tag{CC1}
  \lower16pt\hbox{$\includegraphics[height=1.2cm]{graffles/ccsnakel.pdf}$}
  \eqIH \lower10pt\hbox{$\includegraphics[height=.8cm]{graffles/idncircuit.pdf}$}
  \eqIH \lower16pt\hbox{$\includegraphics[height=1.2cm]{graffles/ccsnaker.pdf}$}
   \end{equation}
in $\IBpoly$ for all $n \in N$. This yields a contravariant

\noindent\begin{minipage}[c]{.75\linewidth}
endofunctor $\coc{(\cdot)}$ on $\IBpoly$ (see also \cite[Rmk~2.1]{Selinger07DaggerCC}): for any $c \: n \to m$, the arrow $\coc{c} \: m\to n$ is defined as on the right.
 \end{minipage}
\begin{minipage}[c]{.25\linewidth}
\vspace{-1cm}\[\includegraphics[height=1cm]{graffles/circuitsnakenospace.pdf}\]
 \end{minipage}
  Using the equational theory of $\IBpoly$, one can show (see \cite[\S4.1]{interactinghopf}) that $\coc{c}$ is just $c$ reflected about the $y$-axis: for example, $\Wmultstar \eqIH \Wcomult$ and $\scalarpstar \eqIH \scalarpop$.

 We list some useful derived laws in $\IBpoly$ below. The proofs are in~\cite[\S4]{interactinghopf}.
  \begin{multicols}{2}\noindent
  \begin{equation}
  \label{eq:ccsliding}
  \tag{CC2}
  \lower10pt\hbox{$\includegraphics[height=1cm,width=2cm]{graffles/ccslidingl.pdf}$}
   \! \eqIH  \! \lower13pt\hbox{$\includegraphics[height=1cm,width=2cm]{graffles/ccslidingr.pdf}$}
   \end{equation}
     \begin{equation}
  \label{eq:ccsliding2}
  \tag{CC3}
  \lower8pt\hbox{$\includegraphics[height=1cm,width=2cm]{graffles/ccsliding2l.pdf}$}
  \! \eqIH \! \lower10pt\hbox{$\includegraphics[height=1cm,width=2cm]{graffles/ccsliding2r.pdf}$}
   \end{equation}
   \end{multicols}
   \smallskip
\begin{multicols}{2}\noindent
\begin{equation}\label{eq:flipscalar}
\lower4pt\hbox{$\includegraphics[height=.5cm]{graffles/scalarop.pdf}$} \eqIH
\lower4.5pt\hbox{$\includegraphics[height=.6cm]{graffles/circuitinvscalar.pdf}$}
\end{equation}
\begin{equation}\label{eq:QFrob}
\lower12pt\hbox{$\includegraphics[height=.9cm]{graffles/QFrob.pdf}$} \eqIH
\lower12pt\hbox{$\includegraphics[height=.9cm]{graffles/QFrob5.pdf}$}
\end{equation}
\end{multicols}
 % \begin{multicols}{2}\noindent
%  \begin{equation}
%  \label{eq:ccsliding}
%  \tag{CC2}
%  \lower10pt\hbox{$\includegraphics[height=1cm,width=2cm]{graffles/ccslidingl.pdf}$}
%   \! \eqIH  \! \lower13pt\hbox{$\includegraphics[height=1cm,width=2cm]{graffles/ccslidingr.pdf}$}
%   \end{equation}
%     \begin{equation}
%  \label{eq:ccsliding2}
%  \tag{CC3}
%  \lower8pt\hbox{$\includegraphics[height=1cm,width=2cm]{graffles/ccsliding2l.pdf}$}
%  \! \eqIH \! \lower10pt\hbox{$\includegraphics[height=1cm,width=2cm]{graffles/ccsliding2r.pdf}$}
%   \end{equation}
%   \end{multicols}
%   \smallskip
%\begin{multicols}{3}\noindent
%\begin{equation}\label{eq:flipscalar}
%\lower4pt\hbox{$\includegraphics[height=.5cm]{graffles/scalarop.pdf}$} \eqIH
%\lower4.5pt\hbox{$\includegraphics[height=.6cm]{graffles/circuitinvscalar.pdf}$}
%\end{equation}
%\begin{equation}\label{eq:QFrob}
%\lower12pt\hbox{$\includegraphics[height=.9cm]{graffles/QFrob.pdf}$} \eqIH
%\lower12pt\hbox{$\includegraphics[height=.9cm]{graffles/QFrob5.pdf}$}
%\end{equation}
%\begin{equation}\label{eq:polyBcc}
%\lower7pt\hbox{$\includegraphics[height=.7cm]{graffles/copolyBcc1.pdf}$}
%\eqIH
%\lower7pt\hbox{$\includegraphics[height=.7cm]{graffles/copolyBcc4.pdf}$}
%\end{equation}
%\end{multicols}

We also record the following lemma; $\nscalarp$ is the $n$-fold product of $\scalarp$.
 \begin{lemma}\label{lemma:xsliding} For any $n,m\in \N$ and circuit $c \in \CD [n,m]$,
 \begin{equation}
   \label{eq:xsliding}
  \lower7pt\hbox{$\includegraphics[height=.7cm]{graffles/circuitCx.pdf}$}
   \quad \eqIH  \quad \lower7pt\hbox{$\includegraphics[height=.7cm]{graffles/circuitxC.pdf}$}
   \end{equation}
 \end{lemma}
 \begin{proof}
The proof is by induction on $c$. For the components in \eqref{eq:SFcalculusSyntax1}, the statement is given for $\Wunit$, $\Wmult$, $\Bcounit$, $\Bcomult$, $\scalar$ and $\circuitX$ by \eqref{eq:scalarwunit}, \eqref{eq:scalarwmult}, \eqref{eq:scalarbcounit}, \eqref{eq:scalarbcomult}, \eqref{eq:scalarmult} and \eqref{eq:scalarmult} respectively. The derivations for $\circuitXop$ and $\coscalar$ are:
     \begin{eqnarray*}
 \lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/circuitxopx.pdf}$}
\! \!\!\eql{\eqref{eq:lcmop}} \!\!\!
 \lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/idcircuit.pdf}$}
\!  \!\!\eql{\eqref{eq:lcm}} \!\!\!
 \lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/circuitxxop.pdf}$}
 \qquad
 \lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/circuitkopx.pdf}$}
 \! \!\!\eql{\eqref{eq:flipscalar}} \!\!\!
 \lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/circuitonekx.pdf}$}
 \! \!\!\eql{\eqref{eq:scalarmult}} \!\!\!
 \lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/circuitxfrattok.pdf}$}
 \! \!\!\eql{\eqref{eq:scalarmult}} \!\!\!
 \lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/circuitxonek.pdf}$}
\!  \!\!\eql{\eqref{eq:flipscalar}} \!\!\!
 \lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/circuitxkop.pdf}$}
 \end{eqnarray*}
Similarly, one can easily check the statement for the remaining cases in \eqref{eq:SFcalculusSyntax2} and \eqref{eq:SFcalculusSyntax3}. The inductive cases of parallel ($\tns$) and sequential ($\poi$) composition of circuits are handled by simply applying the induction hypothesis.
 \end{proof}

%
%\begin{multicols}{2}\noindent
%\begin{equation}\label{eq:QFrob}
%\lower9pt\hbox{$\includegraphics[height=1cm]{graffles/QFrob.pdf}$} =
%\lower9pt\hbox{$\includegraphics[height=1cm]{graffles/QFrob5.pdf}$}
%\end{equation}
%\begin{equation}\label{eq:scalarwcomult}
%\lower8pt\hbox{$\includegraphics[height=.7cm]{graffles/Wcomultpoly.pdf}$}
%=
%  \lower8pt\hbox{$\includegraphics[height=.7cm]{graffles/polyWcomult.pdf}$}
%\end{equation}
%\end{multicols}
%
%\begin{multicols}{2}\noindent
%\begin{equation*}
%%\label{eq:coscalarwmult}
%%\tag{S8}
%\lower11pt\hbox{$\includegraphics[height=.9cm]{graffles/copolyWmult.pdf}$}
%=
%\lower8pt\hbox{$\includegraphics[height=.8cm]{graffles/Wmultcopoly.pdf}$}
%\end{equation*}\noindent
%\begin{equation*}
%\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/copolyBcomult1.pdf}$}
%=
%\lower8pt\hbox{$\includegraphics[height=.8cm]{graffles/copolyBcomult6.pdf}$}
%\end{equation*}
%\end{multicols}




==> source/chapterSFG/backgroundSFG.tex <==
%$\catC[a,b]$ is the set of arrows from $a$ to $b$ in a small category $\catC$, composition of $f \: a \to b$, $g \: b \to c$ is denoted by $f\poi g \: a \to c$. For $\catC$ symmetric monoidal, $\tns$ is the monoidal product and $\sigma_{X,Y} \: X \tns Y \to Y \tns X$ the symmetry for $X,Y \in \catC$. Given $\funF \: \catC_1 \to \catC_2$, $\funF^{\op} \: \catC_1^{\op}\to \catC_2^{\op}$ is the induced functor on the opposite categories of $\catC_1, \catC_2$. If $\catC$ has pullbacks, its span bicategory has the objects of $\catC$ as $0$-cells, spans of arrows of $\catC$ as $1$-cells and span morphisms as $2$-cells. We denote with $\Span{\catC}$ the (ordinary) category obtained by identifying the isomorphic $1$-cells and forgetting the $2$-cells. Dually, if $\catC$ has pushouts, $\Cospan{\catC}$ is the category obtained from the bicategory of cospans.

The categories $\CD$, $\Perm$, $\FC$, $\FCop$ and $\SFGform$ are all PROPs~\cite{MacLane1965,Lack2004a}: a PROP (product and permutation category) is a strict symmetric monoidal category with objects the natural numbers, where $\tns$ on objects is addition. Morphisms between PROPs are identity-on-objects strict symmetric monoidal functors: PROPs and their morphisms form the category $\PROP$.

In this section we introduce the tool kit that we will exploit to give a denotational semantics and an equational theory to $\CD$ (and its sub-PROPs). First, \S\ref{sec:SMTs} presents symmetric monoidal theories as a way of freely constructing PROPs from generators and equations. Then, in \S\ref{ssec:composingPROP} we show how, following~\cite{Lack2004a}, PROPs can be composed together to express richer equational theories.

\subsection{Symmetric Monoidal Theories}\label{sec:SMTs}

A one-sorted \emph{symmetric monoidal theory} (SMT) is a pair $(\Sigma, E)$ where $\Sigma$ is the \emph{signature}: a set of \emph{operations} $o \: n\to m$ with \emph{arity} $n$ and \emph{coarity} $m$. The set of \emph{$\Sigma$-terms} is obtained by composing operations, the identity $\id_1 \: 1\to 1$ and symmetry $\sigma_{1,1} \: 2\to 2$ with $;$ and $\tns$: given $\Sigma$-terms $t \: n\to z$, $u \: z\to m$, $v \: r\to s$, we construct $\Sigma$-terms $t \poi u \: n\to m$ and $t \tns v \: n+r \to m+s$.  The set $E$ of \emph{equations} consists of pairs of $\Sigma$-terms $(t,t' \: n \to m)$.
%
Given an SMT $(\Sigma,E)$, one (freely) obtains a PROP where arrows $n\to m$ are $\Sigma$-terms $n\to m$ modulo the laws of SMC and equations $t=t'$ where $(t,t')\in E$. %There is a graphical representation of terms as string diagrams (see~\cite{Selinger2009}): we call these diagrams \emph{circuits}.

We have already encountered four PROPs freely generated from SMTs with no equations: $\Perm$ is freely generated by the empty theory, $\FC$ by \eqref{eq:SFcalculusSyntax1}, $\FCop$ by \eqref{eq:SFcalculusSyntax2}, and $\CD$ by both \eqref{eq:SFcalculusSyntax1} and \eqref{eq:SFcalculusSyntax2} together---note that components in \eqref{eq:SFcalculusSyntax3} are built-in by definition of SMT.
  %and $\CD$ are the PROPs for the theories having as operations the components , respectively  respectively \eqref{eq:SFcalculusSyntax1} and \eqref{eq:SFcalculusSyntax2}, and no axioms (components in \eqref{eq:SFcalculusSyntax3} are built-in in the definition of SMT).
 Instead, $\SFGform$ is not generated by any SMT, as $\Tr{}(\cdot)$ cannot be expressed as an operation with an arity and coarity.

 Below we introduce three more simple examples of SMT, this time with equations. They constitute the ``building blocks'' for richer theories that will be constructed, in a modular fashion, throughout the paper.
%\begin{itemize}
%\item
\begin{example}[The SMT $(\Sigma_M,E_M)$ of commutative monoids] The signature $\Sigma_M$ consists of multiplication $\Wmult \: 2 \to 1$ and unit $\Wunit \: 0 \to 1$.
% Graphically, the generation of $\Sigma_M$-terms amounts to ``tiling'' $\Wmult$ and $\Wunit$ together with the circuit $\symNet$ (representing $\sigma_{1,1}\: 2 \to 2$) and $\Idnet$ (representing $\id_1 \: 1 \to 1$), in the same way as 2-dimensional diagrams were composed in \S~\ref{sec:SFcalculus}.
Equations $E_M$ assert identity~\eqref{eq:wmonunitlaw}, commutativity~\eqref{eq:wmoncomm} and  associativity~\eqref{eq:wmonassoc}.
 \begin{multicols}{3}\noindent
\begin{equation}
\label{eq:wmonunitlaw}
\tag{A1}
\lower9pt\hbox{$\includegraphics[height=.8cm]{graffles/Wunitlaw.pdf}$}
\!\!\!
=\!
\lower4pt\hbox{$\includegraphics[height=.5cm]{graffles/idcircuit.pdf}$}
\end{equation}
\begin{equation}
\label{eq:wmoncomm}
\tag{A2}
\lower5pt\hbox{$\includegraphics[height=.55cm]{graffles/Wmult.pdf}$}
\!\!
=
\!\!\!\!\!
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Wcomm.pdf}$}
\end{equation}
\begin{equation}
\hspace{-.1cm}\label{eq:wmonassoc}
\tag{A3}
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Wassocl.pdf}$}
\!\!\!\!
=
\!\!\!\!
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Wassocr.pdf}$}
\end{equation}
\end{multicols}
We call $\wmon$ the PROP freely generated from $(\Sigma_M,E_M)$.\footnote{The notation $w$ emphasizes the white colouring of circuits in $\Sigma_M$.} %--- later on, we will use the black coloring for another copy of the same PROP.}
\end{example}

%\item
\begin{example}[The SMT $(\Sigma_C,E_C)$ of commutative comonoids] $\Sigma_C$ consists of operations $\Bcomult\: 1 \to 2$ and $\Bcounit\: 1 \to 0$ and $E_C$ consists of:
\begin{multicols}{3}\noindent
\begin{equation}
\label{eq:bcomonunitlaw}
\tag{A4}
\lower9pt\hbox{$\includegraphics[height=.8cm]{graffles/Bcounitlaw.pdf}$}
\!\!\!
=
\!
\lower4pt\hbox{$\includegraphics[height=.5cm]{graffles/idcircuit.pdf}$}
\end{equation}
\begin{equation}
\label{eq:bcomoncomm}
\tag{A5}
\lower5pt\hbox{$\includegraphics[height=.55cm]{graffles/Bcomult.pdf}$}
\!\!
=
\!\!\!\!
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Bcomm.pdf}$}
\end{equation}
\begin{equation}
\hspace{-.1cm}\label{eq:bcomonassoc}
\tag{A6}
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Bcoassocl.pdf}$}
\!\!\!\!
=
\!\!\!\!
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Bcoassocr.pdf}$}
\end{equation}
\end{multicols}
We call $\bcom$ the PROP freely generated from $(\Sigma_C,E_C)$. Modulo the white vs. black colouring, the circuits of $\bcom$ can be seen as those of $\wmon$ reflected about the $y$-axis. This observation yields that $\bcom \cong \wmon {}^{op}$.
%More generally, for $\T$ a free PROP, $\T^{op}$ can be presented by operations and equations which are those of $\T$ reflected about the $y$-axis.
\end{example}

%\item
\begin{example}[The theory $(\Sigma_R, E_R)$ of multiplication in $\poly$]
Recall that $\poly$ denotes the ring of polynomials over $\field$. The $\Sigma_R$ contains an operation $\scalarp \: 1 \to 1$ for each $p \in \poly$ and $E_R$ consists of the following, where $p_1,p_2$ range over $\poly$.
\begin{multicols}{2}\noindent
\begin{equation}
\label{eq:unitscalar}
\tag{A7}
\lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/unitscalar.pdf}$}
=
\lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/idcircuit.pdf}$}
\end{equation}
\begin{equation}
\label{eq:scalarmult}
\tag{A8}
\lower5pt\hbox{$\includegraphics[height=.6cm]{graffles/polymultl.pdf}$}
=
\lower5pt\hbox{$\includegraphics[height=.6cm]{graffles/polymultr.pdf}$}
\end{equation}
\end{multicols}
We call $\PROPpoly$ the PROP freely generated from $(\Sigma_R, E_R)$.
\end{example}
%\end{itemize}



\begin{comment}
\begin{example}\label{ex:basicSMTs} We provide three examples of PROPs freely generated by SMTs: they will describe equations between the circuit diagrams in~\eqref{eq:SFcalculusSyntax1}.
\begin{itemize}
\item The theory of the adder is the SMT $(\Sigma_M,E_M)$ of commutative monoids. That means, $\Sigma_M$ contains two operation symbols: a multiplication $\Wmult \: 2 \to 1$ and a unit $\Wunit \: 0 \to 1$.
 Graphically, the generation of $\Sigma_M$-terms amounts to ``tiling'' $\Wmult$ and $\Wunit$ together with the circuit $\symNet$ (representing $\sigma_{1,1}\: 2 \to 2$) and $\Idnet$ (representing $\id_1 \: 1 \to 1$), in the same way as 2-dimensional diagrams were composed in \S~\ref{sec:SFcalculus}. Equations $E_M$ assert identity \eqref{eq:wmonunitlaw}, commutativity \eqref{eq:wmoncomm} and associativity \eqref{eq:wmonassoc}.
 \begin{multicols}{3}\noindent
\begin{equation}
\label{eq:wmonunitlaw}
\tag{A1}
\lower9pt\hbox{$\includegraphics[height=.8cm]{graffles/Wunitlaw.pdf}$}
\!\!\!
=\!
\lower4pt\hbox{$\includegraphics[height=.5cm]{graffles/idcircuit.pdf}$}
\end{equation}
\begin{equation}
\label{eq:wmoncomm}
\tag{A2}
\lower5pt\hbox{$\includegraphics[height=.55cm]{graffles/Wmult.pdf}$}
\!\!
=
\!\!\!\!\!
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Wcomm.pdf}$}
\end{equation}
\begin{equation}
\hspace{-.1cm}\label{eq:wmonassoc}
\tag{A3}
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Wassocl.pdf}$}
\!\!\!\!
=
\!\!\!\!
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Wassocr.pdf}$}
\end{equation}
\end{multicols}
We call $\wmon$ the PROP freely generated from $(\Sigma_M,E_M)$.\footnote{The notation $w$ emphasizes the white colouring of circuits in $\Sigma_M$ --- later on, we will use the black coloring for another copy of the same PROP.}

\item The theory of the copier is encoded by the PROP $\bcom$ of (black) cocommutative comonoids, freely generated from the signature consisting of circuits $\Bcomult$, $\Bcounit$ and the following equations.
\begin{multicols}{3}\noindent
\begin{equation}
\label{eq:bcomonunitlaw}
\tag{A4}
\lower9pt\hbox{$\includegraphics[height=.8cm]{graffles/Bcounitlaw.pdf}$}
\!\!\!
=
\!
\lower4pt\hbox{$\includegraphics[height=.5cm]{graffles/idcircuit.pdf}$}
\end{equation}
\begin{equation}
\label{eq:bcomoncomm}
\tag{A5}
\lower5pt\hbox{$\includegraphics[height=.55cm]{graffles/Bcomult.pdf}$}
\!\!
=
\!\!\!\!
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Bcomm.pdf}$}
\end{equation}
\begin{equation}
\hspace{-.1cm}\label{eq:bcomonassoc}
\tag{A6}
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Bcoassocl.pdf}$}
\!\!\!\!
=
\!\!\!\!
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/Bcoassocr.pdf}$}
\end{equation}
\end{multicols}
Modulo the white vs. black colouring, the circuits of $\bcom$ can be seen as those of $\wmon$ ``reflected about the $y$-axis''. This observation yields that $\bcom \cong \wmon {}^{op}$. More generally, for $\T$ a free PROP, $\T^{op}$ can be presented by operations and equations which are those of $\T$, reflected.

\item The PROP $\PROPpoly$ describes multiplication in the polynomial ring $\poly$. It is freely generated from the signature consisting of $\scalarp$ for each $p \in \poly$ and the following equations, where $p_1,p_2$ range over $\poly$.
\begin{multicols}{2}\noindent
\begin{equation}
\label{eq:unitscalar}
\tag{A7}
\lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/unitscalar.pdf}$}
=
\lower5pt\hbox{$\includegraphics[height=.5cm]{graffles/idcircuit.pdf}$}
\end{equation}
\begin{equation}
\label{eq:scalarmult}
\tag{A8}
\lower5pt\hbox{$\includegraphics[height=.6cm]{graffles/polymultl.pdf}$}
=
\lower5pt\hbox{$\includegraphics[height=.6cm]{graffles/polymultr.pdf}$}
\end{equation}
\end{multicols}
\end{itemize}
\end{example}
\end{comment}

%<<<<<<< .mine
%\pippo{I guess that here it should be changed}
%We will sometimes refer to PROPs which arise from SMTs as \emph{equational} PROPs in order to distinguish them from \emph{semantic} PROPs that are defined ``directly'': for instance the PROP of functions $\mathbb{F}$ where arrows $k\to l$ are simply functions $\{0,\dots, k-1\}\to \{0, \dots, l-1\}$.
%=======
%We will sometimes refer to PROPs which arise from SMTs as \emph{equational} PROPs in order to distinguish them\ from \emph{semantic} PROPs that are defined ``directly'': for instance the PROP of functions $\mathbb{F}$ where arrows $k\to l$ are simply functions $\{0,\dots, k-1\}\to \{0, \dots, l-1\}$.\fabio{Consider removing the ``fix terminology'' thing, as equational and semantic are used nowhere later}
%>>>>>>> .r494

Rather than using SMTs, one can also define PROPs ``directly'': an example is the PROP of functions $\mathbb{F}$ where arrows $k\to l$ are functions $\{0,\dots, k-1\}\to \{0, \dots, l-1\}$. There is an isomorphism %$\sem{\wmon}$
 between $\wmon$ and $\F$: to give an arrow $c \: n \to m$ in $\wmon$ is to give the graph of a function  $\{0,\dots, n-1\}\to \{0, \dots, m-1\}$. For instance, $\Wmult \tns \Wunit \: 2 \to 2$ encodes $f \: \{0,1\} \to \{0,1\}$ constant at $0$.
 %Intuitively, $\F$ is a ``concrete'' representation of the theory of commutative monoids; we refer to the morphism $\sem{\wmon}$ as the \emph{denotational semantics} of $\wmon$.

%There is another interesting example of semantic PROP which will be pivotal for our exposition:
%
%\begin{definition} Mat \end{definition}

\subsection{Constructing Richer Theories: Sum and Composition of PROPs}\label{ssec:composingPROP}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Example~\ref{ex:basicSMTs} supplies a canonical set of axioms for the components in \eqref{eq:SFcalculusSyntax1} (and, by duality, for those in \eqref{eq:SFcalculusSyntax3}). However, PROPs $\wmon$, $\bcom$ and $\PROPpoly$ only describe disjoint subsets of \eqref{eq:SFcalculusSyntax1}. What about equations like \lower4pt\hbox{$\includegraphics[height=.5cm]{graffles/bialgl.pdf}$}=\lower6pt\hbox{$\includegraphics[height=.7cm]{graffles/bialgr.pdf}$}, assimilating two ways of expressing the duplication of signal addition?

The SMTs introduced so far are quite simple. Throughout our development, we will deal with more involved cases, which will be convenient to treat as the combination of basic theories. In this section we describe two PROP operations allowing for this modular reasoning: sum and composition.
%We shall understand equations of that kind as arising by the \emph{composition} of $\wmon$, $\bcom$ and $\PROPpoly$, using Lack's theory of composing PROPs~\cite{Lack2004a}.

%As a preliminary step, we describe a more elementary way of combining PROPs, via coproducts.
The sum of PROPs $\T$ and $\PS$ is given by the coproduct $\T + \PS$ in $\PROP$. In order to compute $\T + \PS$, it is useful to note that PROPs are also objects of the coslice category ${\Perm}/\PRO$. Here $\PRO$ is the category of strict monoidal categories (called PROs) with objects the naturals and tensor product on objects addition; morphisms of PROs are strict identity-on-objects monoidal functors. %$\Perm$ is the PRO(P) introduced in \S~\ref{sec:SFcalculus}.
%
Morphisms of PROPs are thus simply morphisms of PROs that preserve the permutation structure. Working in the coslice is quite intuitive: e.g. $\Perm$ is the initial PROP and to compute the coproduct $\T+\PS$ in $\PROP$ one must identify the permutation structures.
When $\T$ and $\PS$ are PROPs freely generated from $(\Sigma_T,E_T)$ and $(\Sigma_S,E_S)$ respectively, it then follows that $\T+\PS$ is the PROP generated by $(\Sigma_T+\Sigma_S,E_T+E_S)$. For instance, $\FC + \FCop$ is simply $\CD$.

\medskip

The sum $\T+\PS$ is the least interesting way of combining PROPs, because there are no equations that express compatibility conditions between $\T$ and $\PS$ when ``interacting'' in $\T+\PS$. Such interactions are common in algebra: for instance, a ring is given by a monoid and an abelian group, subject to equations telling how the former structure distributes over the latter.
%
Another example, which will play a fundamental role in our work, is the PROP of co/commutative \emph{bialgebras}: it consists of $\wmon + \bcom$ quotiented by the following set of equations, expressing the interaction between the monoid and comonoid structures.
\begin{multicols}{2}
\noindent
\begin{equation}
\label{eq:unitsl}
\tag{A9}
\lower7pt\hbox{$\includegraphics[height=.6cm]{graffles/lunitsl.pdf}$}
=
\lower7pt\hbox{$\includegraphics[height=.6cm]{graffles/lunitsr.pdf}$}
\end{equation}\noindent\begin{equation}
\label{eq:unitsr}
\tag{A11}
\lower7pt\hbox{$\includegraphics[height=.6cm]{graffles/runitsl.pdf}$}
=
\lower7pt\hbox{$\includegraphics[height=.6cm]{graffles/runitsr.pdf}$}
\end{equation}
\begin{equation}
\label{eq:bialg}
\tag{A10}
\lower6pt\hbox{$\includegraphics[height=.6cm]{graffles/bialgl.pdf}$}
=
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/bialgr.pdf}$}
\end{equation}
\begin{equation}
\label{eq:bwbone}
\tag{A12}
\lower6pt\hbox{$\includegraphics[height=.5cm]{graffles/unitsl.pdf}$}
=
\lower5pt\hbox{$\includegraphics[width=14pt]{graffles/idzerocircuit.pdf}$} \qquad
\end{equation}
\end{multicols}

 In~\cite{Lack2004a} Lack shows that this interaction arises through a notion of PROP composition, expressed in terms of distributive laws of monads. As shown by Street~\cite{Street_MonadsI}, the theory of monads can be developed in an arbitrary bicategory. In this perspective, small categories are monads in the bicategory $\Span{\Set}$. Similarly, PROPs can be described as monads on $\Perm$ in the bicategory $\mathsf{Prof}(\mathbf{Mon})$ of strict monoidal categories, profunctors and natural transformations~\cite{Lack2004a}.

Now, any two PROPs $\T$ and $\PS$ can be composed via a distributive law $\lambda \colon \PS \poi \T \To \T  \poi \PS$ between the associated monads. $\lambda$ makes $\T \poi  \PS$ into a monad, yielding a PROP whose arrows can be seen as \emph{pairs} $(f,g) \: n \to m$, where $f \: n \to z$ is an arrow of $\T$ and $g \: z \to m$ one of $\PS$.
%
A key observation for our purposes is that the graph of $\lambda$ can be also seen as a set of (directed) equations of the form $(g,f) = (f',g')$. In fact, if $\T$ and $\PS$ are freely generated PROPs then $\T \poi  \PS$ also has a presentation by generators and equations: this is the same as the coproduct $\T +  \PS$, plus the equations encoded by $\lambda$.

As an example, we show how composing $\bcom$ and $\wmon$ yields the PROP of bialgebras. First observe that $\bcom \cong \wmon {}^{\op} \cong \F^{\op}$. Then a distributive law $\lambda \: \wmon \poi \bcom \To \bcom \poi \wmon$ has type $\F \poi \Fop \To \Fop \poi \F$, that is, it maps a pair $p \in \F[n,z]$, $q \in \Fop[z,m]$ to a pair $f \in \Fop[n,z]$, $g \in \F[z,m]$. This amounts to saying that $\lambda$ maps \emph{cospans} $n \tr{p} z \tl{q} m$ to \emph{spans} $n \tl{f} r \tr{g} m$ in $\F$. Defining $n \tl{f} r \tr{g} m$ as the \emph{pullback} of $n \tr{p} z \tl{q} m$ in $\F$ makes $\lambda$ a distributive law~\cite{Lack2004a}. The resulting PROP $\bcom \poi \wmon$ can be presented by operations and equations---those of $\bcom + \wmon$---together with those given by the graph of $\lambda$. One can thus obtain them from pullback squares in $\F$, for instance:
\[
\xymatrix@R=10pt@C=15pt{
& 1 & && & & 1 \ar[dr]^{\Bcounit} &\\
\ar[ur]^{\finVect} 2 & & 0 \ar[ul]_{\initVect_1} & \ar@{|=>}[r] & & \ar[ur]^{\Wmult} 2 \ar[dr]_{\twoBcounit} & & 0 \\
& \ar[ul]^{\initVect_2} 0 \pullbackcorner \ar[ur]_{\id_0} & & && & 0 \ar[ur]_{\ZeronetT} & }
\quad
\lower20pt\hbox{$
\text{yields}
\quad
\Wmult ; \Bcounit = \twoBcounit \poi \ZeronetT
$}
\]
\noindent
where the second diagram is obtained from the pullback by applying the isomorphisms  $\F \cong \wmon$ and
$\Fop \cong \bcom$.
%\fabio{Re-insert explanation of $\finVect$ and $\initVect$ notation?} \pippo{Maybe we can insert it in the notational convention?}
%where $\finVect\: 2 \to 1$ and $\initVect_n \: 0 \to n$ are given, respectively, by finality of $1$ and initiality of $0$ in $\F$, and $\sem{\bcom}$ is the isomorphism $\bcom \cong\Fop$.
In fact, all the equations can be derived from just four pullbacks that yield the four equations \eqref{eq:unitsl}-\eqref{eq:bwbone} given above~\cite{Lack2004a}.

 Therefore $\bcom \poi \wmon$ is the free PROP of (black-white) co/commutative bialgebras. One can consider the SMT of co/commutative bialgebras to be the theory of $\Span{\F} \cong \Fop \poi \F$ and, consequently, that each $c \: n \to m$ in this PROP can be factorised as $c = c_1\poi c_2$, with $c_1 \in \bcom[n,z]$ and $c_2 \in \wmon[z,m]$ for some $z$. 

==> source/chapterSFG/cube.tex <==


\subsection{Soundness and Completeness of $\IBpoly$: the Cube Construction}\label{sec:cube}

Theorem~\ref{thm:semanticsIBpolyIso} and Proposition~\ref{prop:factorisationIH} follow immediately from more general results proved in~\cite[\S 6-10]{interactinghopf}. In this subsection we sketch the proof argument which is interesting in its own right, since it is a \emph{modular} account of the theory of $\IBpoly$. Its components are summarised by the cube diagram~\eqref{eq:cube} below.

\begin{equation}\label{eq:cube}
\tag{\mancube}
\raise50pt\hbox{$
\xymatrix@C=12pt@R=10pt{
& {\ABpoly + \ABpolyop} %\ar[dr]%^{[\varphi_1,\varphi_2]}
\ar[dd]_(.7){\cong}|{\hole}
\ar[dl]%_{[\tau_1,\tau_2]}
\ar[rr]%^{[\sigma_1,\sigma_2]}
& & {\IBpolyw} \ar[dl]%_{\Theta}
\ar[dd]^{\cong} \\
{\IBpolyb} \ar[rr]%^(.7){\Lambda}
\ar[dd]_{\cong}
  & & {\IBpoly} \ar@{.>}[dd]^(.3){\cong} \\
& {\Matpoly+ \Matpolyop} %\ar[dr]%^{[\psi_1,\psi_2]}
\ar[dl]%_{[\iota_1,\iota_2]}
\ar[rr]%^(.45){[\kappa_1,\kappa_2]}|(.55){\hole}
 & & {\SpanMatpoly} \ar[dl]%_{\Phi}
 \\
{\CospanMatpoly} \ar[rr]%^{\Psi}
& & {\SVpoly}
}$}
\end{equation}
%The PROPs that appear in top face of the cube are ``syntactic PROPs'', i.e., they are freely generated from operations and equations. The PROPs that appear in the bottom face are ``semantic PROPs.'' The vertical morphisms are ``denotational semantics'' that map terms to their denotations. For example, as we showed in \S\ref{sec:theorymatr}, $\ABpoly$ is the theory of matrices with entries from the polynomial ring $\poly$, i.e.\ there is an isomorphism of PROPs $\sem{\ABpoly} \: \ABpoly \to \Matpoly$.

The theory $\IBpolyw$ is presented by the equations of $\IBpoly$ (Definition~\ref{def:IBpoly}), but with the two leftmost axioms below replacing  \eqref{eq:bbone} and \eqref{eq:lcmop}.
Dually, $\IBpolyb$ is $\IBpoly$ with the two rightmost axioms below replacing \eqref{eq:wbone} and \eqref{eq:lcm}. As equational theories, $\IBpolyw$ and $\IBpolyb$ are weaker than $\IBpoly$:  all the equations below are derivable in $\IBpoly$~\cite{interactinghopf}.
\begin{multicols}{4}\noindent
\begin{equation*}
\lower9pt\hbox{$\includegraphics[height=.8cm]{graffles/polyWcomult.pdf}$}
\!=\!
  \lower9pt\hbox{$\includegraphics[height=.8cm]{graffles/Wcomultpoly.pdf}$}
\end{equation*}
\begin{equation*}
%\label{eq:coscalarwmult}
%\tag{S8}
\lower11pt\hbox{$\includegraphics[height=.9cm]{graffles/copolyWmult.pdf}$}
\!=\!
\lower8pt\hbox{$\includegraphics[height=.8cm]{graffles/Wmultcopoly.pdf}$}
\end{equation*}\noindent
\begin{equation*}
\lower5pt\hbox{$\includegraphics[height=.8cm]{graffles/Bmultpoly.pdf}$}
\!
=
\!
\lower5pt\hbox{$\includegraphics[height=.9cm]{graffles/derpolyBmult5.pdf}$}
\end{equation*}\noindent
\begin{equation*}
\lower10pt\hbox{$\includegraphics[height=.9cm]{graffles/copolyBcomult1.pdf}$}
\!
=
\!
\lower8pt\hbox{$\includegraphics[height=.8cm]{graffles/copolyBcomult6.pdf}$}
\end{equation*}
\end{multicols}
In fact, $\IBpolyw$ and $\IBpolyb$ are the theories of (i.e. their free PROPs are isomorphic to) $\SpanMatpoly$ and $\CospanMatpoly$, respectively. First we focus on $\IBpolyw$ and $\SpanMatpoly$. Note that pullbacks in $\Matpoly$ exist and are computed as in the category of sets in the equivalent category of finite dimensional $\poly$-vector spaces, since $\poly$ is a principal ideal domain (PID).

Pullbacks give a distributive law of PROPs, and as we explained in \S\ref{ssec:composingPROP}, pullback diagrams ``add equations''  to the theory
$\ABpoly + \ABpolyop$.  Indeed, for each equation of $\IBpolyw$ there is a corresponding ``witnessing'' pullback in $\Matpoly$: this argument confirms the \emph{soundness} of the theory of $\IBpolyw$ for $\Span {\Matpoly}$. The task of demonstrating the
\emph{completeness} of the axioms is more subtle: one has to prove that the axioms are sufficient for deriving \emph{any} equation that arises from a pullback in $\Matpoly$. The proof amounts to showing that linear algebraic manipulations on matrices that are performed when calculating the kernel of a linear transformation %in the category of free $\poly$-modules
can be mimicked graphically in $\IBpolyw$. %Due to space constraints, we refer to our technical report~\cite[\S 6]{interactinghopf} for the details.

Having constructed the isomorphism between $\IBpolyw$ and $\Span{\Matpoly}$, we can use the fact that the transpose operation on matrices induces a duality in $\Matpoly$ to yield the isomorphism between $\IBpolyb$ and $\Cospan{\Matpoly}$.

Now let us again focus on the top face of~\eqref{eq:cube}. It is a pushout diagram in $\PROP$: as only PROPs freely generated by SMTs are involved, this simply amounts to saying that the equational theory of $\IBpoly$ can be presented as the union of the equational theories of $\IBpolyw$ and $\IBpolyb$. An appealing consequence of this construction is that $\IBpoly$ inherits the factorisation properties of both $\IBpolyw$ and $\IBpolyb$. This gives us immediately Proposition~\ref{prop:factorisationIH}.

The final ingredient in the proof Theorem~\ref{thm:semanticsIBpolyIso} is showing that the bottom face of~\eqref{eq:cube} is also a pushout in $\PROP$. We would like to draw the reader's attention to the remarkable fact that subspaces over the \emph{field of fractions} $\frpoly$ of $\poly$ arise from ``glueing'' spans and cospans of $\poly$-matrices. This fact holds for an arbitrary PID and its field of fractions: the proof can be found in~\cite[\S 9]{interactinghopf}.

Summing up, the top and bottom faces of \eqref{eq:cube} are pushouts, and the three rear vertical morphisms are isomorphisms. The universal property of pushouts now ensures that the unique morphism from $\IBpoly$ to $\SVpoly$ is invertible.

%: it is easy to verify that it is the morphism of Definition~\ref{def:SemIB}.

%The provenance of $\IBpoly$ allows us to immediately derive the factorisation properties of Corollary~\ref{prop:factorisationIH}.




==> source/titolo.tex <==

\begin{center}
\vspace{10mm}

{\large\bf TH\`{E}SE}

\vspace{5mm}

{\em en vue d'obtenir le grade de}

\vspace{2.5mm}

{\bf Docteur de l'Universit\'{e} de Lyon}\\[2mm]
{\bf d\'{e}livr\'{e} par l'\'{E}cole Normale Sup\'{e}rieure de Lyon}\\[10mm]
{\bf Discipline~: Informatique}\\[2mm]
{\bf Laboratoire de l'Informatique du Parall\'{e}lisme}\\[2mm]
{\bf \'{E}cole Doctorale en Informatique et Math\'{e}matiques de Lyon}\\[2mm]


\vspace{8mm}
{\em pr\'{e}sent\'{e}e et soutenue publiquement le 5 Octobre 2015}\\
{\em par Monsieur Fabio ZANASI}\\

\vspace{20mm}
%\vfill

{
    \sffamily\bfseries\LARGE
    \begin{center}
    \line(1,0){250}
    
    \vspace{2mm}
      \textbf{\large Interacting Hopf Algebras} \\
      \textsc{\normalsize the theory of linear systems}
    \vspace{1mm}
    
          \line(1,0){250}
\end{center}%
  }%
%\vfill

\vspace{3cm}
\small

\end{center}

\begin{tabular}{lllll}
\textit{Directeur de th\`{e}se~:} &M. &Daniel & HIRSCHKOFF & \\[2mm]
%\multicolumn{4}{c}{\qquad \textit{Apr\`{e}s l'avis de~:}}\\[2mm]
\textit{Apr\`{e}s l'avis de~:}  & M. &Samson &  ABRAMSKY & \\
                & M. &Pierre-Louis &  CURIEN &\\
                & M. &Peter &  SELINGER & \\[2mm]
%\multicolumn{4}{c}{\qquad \textit{Devant le jury compos\'{e}e de~:}}\\[2mm]
\textit{Devant le jury compos\'{e}e de~:}      &M. &Samson &  ABRAMSKY &\textit{Rapporteur}\\
                & M. &Filippo &  BONCHI &\textit{Co-encadrant}\\
                & M. &Pierre-Louis &  CURIEN &\textit{Rapporteur}\\
		&M. &Daniel  & HIRSCHKOFF &\textit{Directeur}\\
                &M. &Samuel  & MIMRAM &\textit{Examinateur}\\
                &M. & Prakash &  PANANGADEN &\textit{Examinateur}
\end{tabular}
\thispagestyle{empty}
\makeatother

\newpage\null\thispagestyle{empty}\newpage
% \cleardoublepage

%\title{Interacting Hopf Algebras \\ \textsc{\small the Theory of Linear Systems}}
%\author{Fabio Zanasi}

%\date{1 April 1993\thanks{First drafted on 29 February 1992}}
%\maketitle 

==> source/titoloOLD.tex <==

\begin{center}
\large{\sc \textbf{ - \'{E}cole normale sup\'{e}rieure de Lyon -}}\\
Laboratoire de l'Informatique du Parall\'{e}lisme - UMR5668 - LIP

\vspace{8mm}

{\large\bf TH\`{E}SE}

\vspace{5mm}

{\em \small en vue d'obtenir le grade de}

\vspace{2.5mm}

{\bf Docteur de l'Universit\'{e} de Lyon, d\'{e}livr\'{e} par}\\[2mm]
 {\bf l'\'{E}cole Normale Sup\'{e}rieure de Lyon} \\[2mm]
{\bf Sp\'{e}cialit\'{e}~: Informatique}\\[2mm]


\vspace{4mm}
{\em \small au titre de l'\'{E}cole Doctorale Informatique et Math\'{e}matiques}\\

\vspace{4mm}

{\em \small pr\'{e}sent\'{e}e et soutenue publiquement le 5 Octobre 2015 par}

\vspace{5mm}

{\large Fabio Zanasi}

\vspace{10mm}
%\vfill

{
    \sffamily\bfseries\LARGE
    \begin{center}
      \textbf{Interacting Hopf Algebras} \\
      \textsc{\normalsize the theory of linear systems}
\end{center}%
  }%
%\vfill



\vspace{1.5cm}
\small

\end{center}
\begin{tabular}{llll}
\phantom{\textit{Directeurs de th\`{e}se~:}} &\phantom{Filippo} & \phantom{BONCHI} & \\
%&Daniel & HIRSCHKOFF & \\[3mm]
%\textit{Devant la commission d'examen form\'{e}e de~:}
\multicolumn{4}{c}{\qquad \textit{Commission d'examen form\'{e}e de~:}}\\[2mm]
                & Samson &  ABRAMSKY &\textit{Rapporteur}\\
                & Filippo &  BONCHI &\textit{Directeur}\\
                & Pierre-Louis &  CURIEN &\textit{Rapporteur}\\
		&Daniel  & HIRSCHKOFF &\textit{Directeur}\\
                &Samuel  & MIMRAM &\textit{Examinateur}\\
                & Prakash &  PANANGADEN &\textit{Examinateur}\\
                & Peter &  SELINGER &\textit{Rapporteur}\\
\end{tabular}
\thispagestyle{empty}
\makeatother

\newpage\null\thispagestyle{empty}\newpage
% \cleardoublepage

%\title{Interacting Hopf Algebras \\ \textsc{\small the Theory of Linear Systems}}
%\author{Fabio Zanasi}

%\date{1 April 1993\thanks{First drafted on 29 February 1992}}
%\maketitle 
